General method for atomistic spin-lattice dynamics with first principles accuracy

We present a computationally efficient general first-principles based method for spin-lattice simulations for solids. Our method is based on a combination of atomistic spin dynamics and molecular dynamics, expressed through a spin-lattice Hamiltonian where the bilinear magnetic term is expanded to second order in displacement, and all parameters are computed using density functional theory. The effect of first-order spin-lattice coupling on the magnon and phonon dispersion in bcc Fe is reported as an example, and is seen to be in good agreement with previous simulations performed with an empirical potential approach. In addition, we also illustrate the abilities of our method on a more conceptual level, by exploring dissipation-free spin and lattice motion in small magnetic clusters (a dimer, trimer and quadmer). Our method opens the door for quantitative description and understanding of the microscopic origin of many fundamental phenomena of contemporary interest, such as ultrafast demagnetization, magnetocalorics, and spincaloritronics.

==> konstig_ref.tex <==
@article{Soddemann2003,
abstract = {We discuss dissipative particle dynamics as a thermostat to$\backslash$nmolecular dynamics, and highlight some of its virtues: (i) universal$\backslash$napplicability irrespective of the interatomic potential; (ii) correct and$\backslash$nunscreened reproduction of hydrodynamic correlations; (iii) stabilization of$\backslash$nthe numerical integration of the equations of motion; and (iv) the avoidance of$\backslash$na profile bias in boundary-driven nonequilibrium simulations of shear flow.$\backslash$nNumerical results on a repulsive Lennard-Jones fluid illustrate our arguments.$\backslash$n},
annote = {NULL},
author = {Soddemann, T. and D$\backslash$$\backslash$"unweg, B. and Kremer, K.},
doi = {10.1103/PhysRevE.68.046702},
file = {:Users/johan/Work/Articles/Physrev/PhysRevE.68.046702.pdf:pdf},
isbn = {1063-651X
1095-3787},
issn = {1063-651X},
journal = {Phys. Rev. E},
number = {4},
pages = {046702},
title = {{Dissipative particle dynamics: A useful thermostat for equilibrium and nonequilibrium molecular dynamics simulations}},
url = {http://pre.aps.org/abstract/PRE/v68/i4/e046702},
volume = {68},
year = {2003}
}
